QUEST: QUantum-Enhanced Shared Transportation

We introduce ``Windbreaking-as-a-Service'' (WaaS) as an innovative approach to shared transportation in which larger ``windbreaker'' vehicles provide aerodynamic shelter for ``windsurfer'' vehicles, thereby reducing drag and fuel consumption. As a computational framework to solve the large-scale matching and assignment problems that arise in WaaS, we present \textbf{QUEST} (Quantum-Enhanced Shared Transportation). Specifically, we formulate the pairing of windbreakers and windsurfers -- subject to timing, speed, and vehicle-class constraints -- as a mixed-integer quadratic problem (MIQP). Focusing on a single-segment prototype, we verify the solution classically via the Hungarian Algorithm, a Gurobi-based solver, and brute-force enumeration of binary vectors. We then encode the problem as a Quadratic Unconstrained Binary Optimization (QUBO) and map it to an Ising Hamiltonian, enabling the use of the Quantum Approximate Optimization Algorithm (QAOA) and other quantum and classical annealing technologies. Our quantum implementation successfully recovers the optimal assignment identified by the classical methods, confirming the soundness of the QUEST pipeline for a controlled prototype. While QAOA and other quantum heuristics do not guarantee a resolution of the fundamental complexity barriers, this study illustrates how the WaaS problem can be systematically translated into a quantum-ready model. It also lays the groundwork for addressing multi-segment scenarios and potentially leveraging quantum advantage for large-scale shared-transportation instances.

==> listing.tex <==
\section*{Listings}

\begin{lstlisting}[language=Python, caption={Hungarian Algorithm for single-segment assignment}, label={lst:hungarian}]
from scipy.optimize import linear_sum_assignment

def find_maximum_matching(cost_matrix):
    # Apply the Hungarian algorithm
    row_ind, col_ind = linear_sum_assignment(cost_matrix)
    # The optimal assignment is given by the indices of row_ind and col_ind
    optimal_value = cost_matrix[row_ind, col_ind].sum()
    return row_ind, col_ind, optimal_value
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={Exhaustive QUBO search for small instances}, label={lst:bruteforce}]
import itertools
import numpy as np

# A_2D is the QUBO matrix (n^2 x n^2)
min_qubo_value = None
optimal_vector = None
all_possible_vectors = itertools.product([0,1], repeat=n*n)

for vector in all_possible_vectors:
    x = np.array(vector)
    qubo_value = x @ A_2D @ x  # x^T A_2D x

    if (min_qubo_value is None) or (qubo_value < min_qubo_value):
        min_qubo_value = qubo_value
        optimal_vector = x

print("Optimal QUBO Value:", min_qubo_value)
print("Optimal Vector:", optimal_vector)
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={Constructing the QUBO matrix with penalties}, label={lst:QUBO-construction}]
lambda_3 = 650000
A = np.zeros((n, n, n, n))

for i in range(n):
    for j in range(n):
        for l in range(n):
            for m in range(n):
                if i == j:
                    if l == m:
                        # Diagonal: cost of (surfer=i, breaker=l) minus penalty
                        A[i, j, l, m] = cost_matrix[i, l] - 2*lambda_3
                    else:
                        # Surfer i assigned to two different breakers => penalty
                        A[i, j, l, m] = lambda_3
                else:
                    if l == m:
                        # Two different surfers assigned to breaker l => penalty
                        A[i, j, l, m] = lambda_3
                    else:
                        A[i, j, l, m] = 0

# Reshape into a 2D matrix (n^2 x n^2)
A_2D = np.zeros((n*n, n*n))
for i in range(n):
    for j in range(n):
        A_2D[i*n:(i+1)*n, j*n:(j+1)*n] = A[i, j]
\end{lstlisting}

\begin{lstlisting}[language=Python, caption={Interpreting the final QUBO solution}, label={lst:QUBO-interpretation}]
# Suppose 'optimal_vector' is the minimizer of x^T A_2D x
solution_matrix = optimal_vector.reshape((n, n))
matching = {}
assigned_breakers = set()

for surfer in range(n):
    assigned = False
    for breaker in range(n):
        if solution_matrix[surfer][breaker] == 1:
            if breaker not in assigned_breakers:
                matching[surfer] = breaker
                assigned_breakers.add(breaker)
                assigned = True
                break
    if not assigned:
        print(f"Surfer {surfer} could not be assigned to any Breaker.")

print("\nSurfer-Breaker Assignments:")
for surfer, breaker in matching.items():
    print(f"Surfer {surfer} -> Breaker {breaker}")
\end{lstlisting}
